QR Sort: A Novel Non-Comparative Sorting Algorithm

In this paper, we introduce and prove QR Sort, a novel non-comparative integer sorting algorithm. This algorithm uses principles derived from the Quotient-Remainder Theorem and Counting Sort subroutines to sort input sequences stably. QR Sort exhibits the general time and space complexity $\mathcal{O}(n+d+\frac{m}{d})$, where $n$ denotes the input sequence length, $d$ denotes a predetermined positive integer, and $m$ denotes the range of input sequence values plus 1. Setting $d = \sqrt{m}$ minimizes time and space to $\mathcal{O}(n + \sqrt{m})$, resulting in linear time and space $\mathcal{O}(n)$ when $m \leq \mathcal{O}(n^2)$. We provide implementation optimizations for minimizing the time and space complexity, runtime, and number of computations expended by QR Sort, showcasing its adaptability. Our results reveal that QR Sort frequently outperforms established algorithms and serves as a reliable sorting algorithm for input sequences that exhibit large $m$ relative to $n$.

==> backups.tex <==
\subsection{Nested QR Sort}\label{implementation_section_nested}
With the recommended implementation, QR Sort conducts two stable sorts by the remainder and quotient keys $R$ and $Q$ using Counting Sort such that the final sorted sequence $S' = f(f(S, R), Q)$. Another implementation option exists where, after computing $S^{(1)} = f(S, R)$ with Counting Sort, we then compute $S' = f(S^{(1)}, Q)$ using a nested QR Sort. The nested QR Sort calculates remainder and quotient keys $R^{(1)}$ and $Q^{(1)}$ for $Q$, and computes $S^{(2)} = f(S^{(1)}, R^{(1)})$ using Counting Sort. Then, the nested QR Sort calculates the remainder and quotient keys $R^{(2)}$ and $Q^{2}$ for $Q{(1)}$, and computes $S^{(3)} = f(S^{(2)}, R^{(2)})$ using Counting Sort. This process repeats $a$?? times, until sorting $S^{(a)} = f(S^{(a,R)},R^{(a-1)}$ and then finally $S' = S^{(a,Q)} = f(S^{(a,R)}),Q^{(a-1)}$ using Counting Sort both times.

In summary, let Eq. (\ref{equation_Qa}) and Eq. (\ref{equation_Ra}) define $q_i^{(j)}$ and $r_i^{(j)}$, respectively, for each $s_i$ in $S$, and let $j$ represent the nested QR sort iteration. Then, we compute $S'$ with Eq. (\ref{equation_nested_QR}), using Counting Sort as the stable sorting algorithm for each $f(S^{(j)},R^{(j)})$ subroutine.

\begin{equation}\label{equation_Qa}
q_i^{(j)} =  \lfloor \frac{s_i}{d^j} \rfloor = \lfloor \frac{q_i^{(j-1)}}{d} \rfloor
\end{equation}

\begin{equation}\label{equation_Ra}
r_i^{(j)} = q_i^{(j)} \Mod{d}
\end{equation}

\begin{equation}\label{equation_nested_QR}
S' = f(f( \ldots f(f(S, R^{(1)}), R^{(2)}) \ldots, R^{(a)}) Q^{(a)})
\end{equation}

Using a nested QR Sort implementation provides the potential to decrease time complexity.



* Something about how the other optimizations are for specific use cases, but this one can be tuned to any user's specific scenario by finding optimal tunable parameters. We provide them more arguments to do this. 

One option:
until the user stops it, or all quotient keys $Q^{(a)}$ equal zero, implying that the most recently sorted sequence $S^{(a)}$ equals $S'$. 
DEFINE A???

changing d is another option

* Downsides to this:
decrease theoretical time complexity, but computing additional remainders and quotients negatively degrades performance as they are themselves expensive operations 
The more times we do this the more we perform expensive computations which in the end may not reflect the good time complexity

* Figure out what all this is and where to fit it:

If we perform a single-nested QR Sort with $d=n$, it achieves the time complexity of $\mathcal{O}(n + \frac{k}{n^2})$. In the worst case for a nested QR Sort, it performs a remainder sort on the input array values, then another remainder sort on the quotient key values, followed by a quotient sort on the reduced quotient key values. An $m$-nested QR Sort achieves the time complexity of $\mathcal{O}((n+d)*m + \frac{k}{d^m})$.

By repetitively dividing the quotient key values by $d$ in the nested QR Sort operations, we find that the largest possible value for $m$ equals $\lfloor \log_d(k) \rfloor$. At this point, every key reduces to zero, which triggers the end-early condition of QR Sort as noted in Section \ref{algorithms_section_qr_sort}. If we assign $m$ to $\lfloor \log_d(k) \rfloor$ in the generalized time complexity, it develops into $\mathcal{O}((n+d)*\log_d(k) + \frac{k}{d^{\log_{d}(k)}})$ which simplifies to $\mathcal{O}((n+d)*log_d(k))$. This specific instance of the generalized QR Sort achieves the same time complexity of Radix Sort and performs identical operations at each iteration. We interpret each nested QR Sort operation as a Radix Sort of the $m$-th digit in the base $d$ number system. 

For nested QR Sort operations, the value for $d$ need not remain constant. Let $D$ represent the ordered sequence of user-selected divisors used to compute the remainder and quotient keys in each nested QR Sort. We further generalize the time complexity of QR Sort to:

\begin{equation*}
\mathcal{O}\left(n\cdot\lvert D\rvert + \sum_{d\in D} d +k\prod_{d\in D}d^{-1}\right)
\end{equation*}

If we assume $1 < d < k$ for each $d\in D$, we bound the sequence length with the inequality $1 <\lvert D\rvert < \log_2(k)$. We require further research and detailed experimental analysis to find the optimal input parameters needed to guarantee nested QR Sort performance improvements.


\begin{figure}
    \centering
    \includegraphics[scale=.45]{figure_2.png}
    \caption{Illustration of Radix Sort Applied to an Integer Array. This visual demonstrates the step-by-step process of sorting the array by each digit.}
    \label{fig:radix_fig}
\end{figure}



\subsection{Radix Sort Comparison}\label{results_and_discussion_section_radix_sort_comparison}
In Figure \ref{fig4}, Our analysis indicates that Radix Sort outperforms QR Sort for array lengths less than 2,350. We link the subsequent performance improvement of QR Sort to its hyperbolic term, $\frac{k}{n}$, in its time complexity. In extreme cases, this term adversely affects the computational performance of QR Sort as illustrated by the initial downward graphic trend. However, this effect diminishes with increasing array lengths as the algorithm approaches linear time $\mathcal{O}(n)$. Based on these observations and the ones concluded in Figure \ref{fig3}, we surmise that QR Sort maintains superior performance over Radix Sort for arbitrary array lengths beyond their plotted intersection.   

We developed QR Sort, a novel stable integer sorting algorithm, to reduce the number of sorting iterations and intensive division and modulo operations required to extract the digit keys in Radix Sort. 


When $d$ equals $n$, this expression simplifies to $\mathcal{O}(n+\frac{k}{n})$, suggesting that QR Sort converges to $O(n)$ faster than Radix Sort. Some implementations of Radix Sort preform operations to extract the digit keys that result in exponentially growing terms \cite{gries_radix_sort} and leave Radix Sort susceptible to arithmetic overflow errors. QR Sort serves as a safer alternative to Radix Sort \cite{gries_radix_sort} as it contains no such growing terms. We present QR Sort pseudo code in Pseudo Code in \ref{psuedo_code_qr_sort}.

Contrary to Radix Sort, which executes $\mathcal{O}(\log_b(k))$ sorting iterations, QR Sort invokes at most two. This reduction tends to produce larger keys, which in turn require additional bins to process. However, the improved computational performance justifies the greater memory consumption in systems with ample space. We explore scenarios where the number of bin accesses in QR Sort exceeds the total number of Radix Sort arithmetic operations but articulate their rarity section \ref{results_and_discussion_section_radix_sort_comparison}. 

\<QR Sort omits the sort on $S'$ by $Q$ if the largest quotient equals zero as this infers that the initial remainder sort already sorted $S$. We prove this result in.\>

We also observe distinct performance spikes in QR Sort and Radix Sort in plots A and B, near array lengths 50,000 and 500,000 respectively. Both algorithms demonstrate multiple performance fluctuations of this nature until the array length surpasses $k$. We attribute this behavior to the dynamic combined influence between the varying array lengths and $k$ values, coupled with the impact of the floor function on the computational complexity of these algorithms, a method known to cause sharp variations in graphical representations of data.



\begin{theorem}\label{O(n)_derivation} 
When QR Sort just executes a remainder sort with no subsequent quotient sort, the optimal divisor $d = m+1$ is used (see Theorem \ref{OptimalDivisorTheorem_R}), and the input sequence length $n$ is proportional to $m$ (defined in \ref{definition_2}), the time and space complexity of QR Sort evaluates to linear time, or $\mathcal{O}(n)$.
\end{theorem}

\begin{proof}
Let QR Sort only perform a remainder sort with no subsequent quotient sort. Also, let the divisor $d = m+1$ (see Theorem \ref{OptimalDivisorTheorem_R}). Then, we begin with the reduced time and space complexity of QR Sort presented in Theorem \ref{OptimalDivisorTheorem_R} for instances when only the remainder sort is performed: $\mathcal{O}(n + m)$. 

Next, let the input sequence length $n$ be proportional to $m$ (defined in \ref{definition_2}). Then, we can define the relationship between $n$ and $m$ in Eq. (\ref{n_m_proprtional}), where $c$ is some constant. 

\begin{equation}\label{n_m_proprtional}
m = c * n
\end{equation}

Plugging Eq. (\ref{n_m_proprtional}) into $\mathcal{O}(n + m)$ yields:

\begin{equation}\label{n_m_proprtional}
\mathcal{O}(n + m) = \mathcal{O}(n + c * n) = \mathcal{O}(n)
\end{equation}
\end{proof}




\subsection{Comparison of QR Sort to Radix Sort}\label{analyses_section_comparison_to_radix_sort}

Next, we present an in-depth analysis that contrasts the computational efficiencies of QR Sort and Radix Sort. <Why? Or maybe explain why after the explanation of Radix Sort>

Least Significant Digit Radix Sort, or Radix Sort for short, constitutes another stable integer sorting algorithm \cite{cormen_et_al, gries_radix_sort}. Radix Sort represents each $v$ in $S$ as $v - \min(S)$, and then invokes a stable sort using the least significant digit of each $v - \min(S)$ as representative keys. Next, Radix Sort performs a stable sort on the resulting sequence $S'$, utilizing the next least significant digit of each element as the representative keys. This repeats until it exhausts the remaining digits. Figure \ref{fig:radix_fig} depicts the execution of Radix Sort on an integer array, and delineates the outcomes of each stable sorting iteration.

Radix Sort enables sorting sequences with elements expressed in both decimal and other positive number systems. Let $b$ denote the base of the number system Radix Sort employs on $S$. The implementation of Radix Sort in \cite{gries_radix_sort} uses Counting Key Sort as the stable sorting algorithm with $\lfloor log_b(k) \rfloor$ iterations, each exhibiting a time complexity of $\mathcal{O}(n+b)$ \cite{cormen_et_al}. As such, the overall time complexity of this implementation equals $\mathcal{O}((n+b)*log_b(k))$ \cite{gries_radix_sort}. Then, if $b=n$, the overall time complexity simplifies to $\mathcal{O}(n*log_n(k))$ and decreases exponentially as $n$ increases. 

\<This instance of Radix Sort also exhibits a spacial complexity $\mathcal{O}(n)$ independent of $k$.\> 
\<However, an implementation caveat of Radix Sort lies in its susceptibility to overflow errors caused by the exponential growth of the radix term in scenarios sorting arrays with large $k$ values.\> 

To conduct this comparison, we ran one SortTester\_C experiments, where the maximum element value $m$ in array $A$ was 150,000,000. <We chose this particular value of $k$ as it marks a point where Counting Sort exhibits significant performance inefficiencies. - this doesn't show up in your prev. figure at all though? Could you use one of those values instead? Or explain this further? Again, the minimum and maximum array lengths, $min\_length$ and $max\_length$, were set to 0 and 1,000,000, respectively. <Why?> SortTester\_C generated a plot of the natural logarithm of the average computational units for QR Sort and Radix Sort by array length $n$. 

<We also need to say something about for Radix Sort b = n and QR Sort d = n>

Like QR Sort, Radix Sort uses Counting Sort subroutines to sort its keys. Radix Sort invokes $\mathcal{\log_n{m}}$ Counting Sort subroutines. As $n$ grows, the total number of subroutines invoked decreases, causing sudden dips in the plots of the number of computational units expended by Radix Sort (Figure /ref{}a-b?).

 We also observe distinct performance spikes in QR Sort and Radix Sort in plots A and B, near array lengths 50,000 and 500,000 respectively. Both algorithms demonstrate multiple performance fluctuations of this nature until the array length surpasses $k$. We attribute this behavior to the dynamic combined influence between the varying array lengths and $k$ values, coupled with the impact of the floor function on the computational complexity of these algorithms, a method known to cause sharp variations in graphical representations of data. Based on these findings, Figure \ref{fig3} leads us to conclude the superiority of QR Sort in consistent and reliable performance among the other algorithms tested in these scenarios. 

 In this paper, we introduce QR Sort, a novel non-comparative integer sorting algorithm. This algorithm uses principles derived from the Quotient Remainder Theorem and Counting Sort subroutines to sort input sequences stably. QR Sort exhibits a time and space complexity of $\mathcal{O}(n+d+\frac{m}{d})$, where $n$ denotes the input sequence length, $d$ denotes a predetermined positive integer, and $m$ denotes the range of input sequence values plus 1. Furthermore, when $n \propto m$, QR Sort attains a linear time and space complexity of $\mathcal{O}(n)$. Our results reveal that QR Sort frequently outperforms established algorithms and serves as a reliable sorting algorithm for input sequences that exhibit larger input sequence element ranges. Additionally, we offer thorough details that surpass the usual depth found in typical sorting algorithm papers that highlight the robustness of our approach and algorithm. We accomplish this by showcasing implementation optimizations, comprehensive pseudo code, and rigorous proofs.




 % Static / Dynamic 

\subsection{Minimizing Computations}\label{minimizing_computations}

Recall that QR Sort sorts both the remainder and quotient keys unless $\lfloor\frac{m}{d}\rfloor = 0$, in which case only the remainder keys are sorted and the quotient key sort is bypassed.
To minimize the computations expended by QR Sort, divisor $d$ must be selected by using both Theorems \ref{OptimalDivisorTheorem_RQ} and \ref{theorem_4_bypass_quotiet} under the conditions expressed in the piecewise function in Eq. (\ref{pick_m}). Specifically, the user must select values for the constants $x$ and $y$ based on their implementation of QR Sort.

\begin{equation}\label{pick_m}
d = 
\begin{cases} 
\sqrt{m} & \text{for } x \cdot n + y \leq m \\
m + 1 & \text{for } x \cdot n + y > m
\end{cases}
\end{equation}

\begin{equation}\label{pick_x}
x = -\frac{(a_r - a_q)}{b_r}
\end{equation}

\begin{equation}\label{pick_y}
y = \frac{b_q^2}{b_r^2} - \frac{(c_r - c_q)}{b_r}
\end{equation}

Specifically, the user must select values for the constants $x$ and $y$ at the transition point of the piecewise function using Eq. (\ref{pick_x}) and (\ref{pick_y}), respectively, based on their implementation of QR Sort. In both expressions, the $a$, $b$, and $c$ denote constants that encapsulate the number of computations of $n$ and $m$. We express the number of computations expended by an implementation of QR Sort when both the remainder and quotient key sorts are performed as $a_q n + b_q \sqrt{m} + c_q$. Likewise, we present the number of computations expended by a specific implementation of QR Sort when only the remainder key sort is performed and the quotient key sort is bypassed as $a_r n + b_r m + c_r$. With this framework for expressing number of computations expended by QR Sort, we present a proof for Eq. (\ref{pick_x}) and (\ref{pick_y}) in Appendix \ref{appendix_params}.


 The user may find these values using static or dynamic analysis of a specific QR Sort implementation. Static analysis may abstract away key processes and details in high-level code, like compiler optimizations affecting $x$ and $y$. Dynamic analysis may return more accurate experimental values, though results may differ on other computing platforms. 

 Comparison-based algorithms only depend on $n$, whereas non-comparative algorithms depend on both $n$ and $m$. Non-comparative algorithms achieve near-linear sorting times when $m$ remains small. In contrast, comparison-based algorithms, with the lower bound time complexity $\mathcal{O}(n\log{n})$, remain independent of $m$ \cite{cormen_et_al}. As such, non-comparative algorithms outperform comparison-based algorithms with smaller $m$. However, as $m$ grows, the number of computations increases for non-comparative algorithms, degrading performance. As shown in Table \ref{tab:complexity_comparison}, Merge Sort and Quicksort constitute comparison-based algorithms, while QR Sort constitutes a non-comparative algorithm. In our results, QR Sort outperforms Merge Sort and Quicksort. However, we expect both to outperform QR Sort when $m$ grows to a large enough value. 


%\section{Acknowledgements}\label{acknowledgements}
%We thank the Johns Hopkins University Applied Physics Laboratory for providing the publication fee. The content is solely the responsibility of the authors and does not represent the official views of the funding institution.


  In this paper, we introduce and prove QR Sort, a novel non-comparative integer sorting algorithm. This algorithm uses principles derived from the Quotient-Remainder Theorem and Counting Sort subroutines to sort input sequences stably. QR Sort exhibits a time and space complexity of $\mathcal{O}(n+d+\frac{m}{d})$, where $n$ denotes the input sequence length, $d$ denotes a predetermined positive integer, and $m$ denotes the range of input sequence values plus 1. We prove that when $m \leq \mathcal{O}(n^2)$, QR Sort attains a linear time and space complexity of $\mathcal{O}(n)$. We provide implementation optimizations for minimizing the time and space complexity, runtime, and number of computations expended by QR Sort, showcasing its adaptability.  Our results reveal that QR Sort frequently outperforms established algorithms and serves as a reliable sorting algorithm for input sequences that exhibit large $m$ relative to $n$. 
